Combined collider constraints on neutralinos and charginos

Searches for supersymmetric electroweakinos have entered a crucial phase, as the integrated luminosity of the Large Hadron Collider is now high enough to compensate for their weak production cross-sections. Working in a framework where the neutralinos and charginos are the only light sparticles in the Minimal Supersymmetric Standard Model, we use gambit to perform a detailed likelihood analysis of the electroweakino sector. We focus on the impacts of recent ATLAS and CMS searches with 36 fb$^{-1}$ of 13 TeV proton-proton collision data. We also include constraints from LEP and invisible decays of the $Z$ and Higgs bosons. Under the background-only hypothesis, we show that current LHC searches do not robustly exclude any range of neutralino or chargino masses. However, a pattern of excesses in several LHC analyses points towards a possible signal, with neutralino masses of $(m_{\tilde{\chi}_1^0}, m_{\tilde{\chi}_2^0}, m_{\tilde{\chi}_3^0}, m_{\tilde{\chi}_4^0})$ = (8-155, 103-260, 130-473, 219-502) GeV and chargino masses of $(m_{\tilde{\chi}_1^{\pm}}, m_{\tilde{\chi}_2^{\pm}})$ = (104-259, 224-507) GeV at the 95% confidence level. The lightest neutralino is mostly bino, with a possible modest Higgsino or wino component. We find that this excess has a combined local significance of $3.3\sigma$, subject to a number of cautions. If one includes LHC searches for charginos and neutralinos conducted with 8 TeV proton-proton collision data, the local significance is lowered to 2.9$\sigma$. We briefly consider the implications for dark matter, finding that the correct relic density can be obtained through the Higgs-funnel and $Z$-funnel mechanisms, even assuming that all other sparticles are decoupled. All samples, gambit input files and best-fit models from this study are available on Zenodo.

==> comparison.tex <==
\input{R1_template.tex}

\newcommand\dd{{\rm d}}

\newcommand\paperitem[1]{\noindent \textcolor{darkred}{- #1}\\}
\renewcommand{\dbltopfraction}{0.9}     % fit big float above 2-col. text
\renewcommand{\textfraction}{0.07}      % allow minimal text w. figs

% Shorthand commands for the most cumbersome input parameters
\newcommand\msf{m_{\tilde{f}}}
\newcommand\msfsq{m_{\tilde{f}}^2}
\newcommand\MHusq{M_{H_u}^2}
\newcommand\MHdsq{M_{H_d}^2}

\begin{document}

\section{Comparison with literature results}

To the best of our knowledge, our present study is the first global fit of the MSSM7. Benchmark points obeying the relic density constraint were obtained via a simple MSSM7 scan of 5000 random points in~\cite{darksusy}. Points from a random scan that give the correct relic density whilst remaining consistent with LEP limits on the chargino mass and Higgs exclusion limits were presented in~\cite{BMSSM}, where this paper predates the Higgs discovery. A random scan for points obeying the relic density constraint was also performed in~\cite{IC22Methods}, with an emphasis on determining the impact of the IceCube neutrino telescope. Finally, MSSM7 points, obtained via an adaptative grid scan, consistent with a variety of collider constraints (including a Higgs mass of 125 GeV) plus a one-sided relic density limit and the Xenon 100 limit on the SI WIMP-proton cross-section were shown in the $m_{\tilde{\chi}_1^0}$-$\sigma_{\text{p,SD}}$ and $m_{\tilde{\chi}_1^0}$-$\sigma_{\text{p,SI}}$ planes in~\cite{Adrian-Martinez:2013ayv}. 

None of these studies are directly comparable to the present study for a variety of reasons. Firstly, and most importantly, the results are presented in the form of either benchmark point tables, or simple plots of non-excluded models, with no attempt to give a profile likelihood function. The \emph{shape} of the allowed regions is therefore unrelated to the shapes that we obtain. Secondly, the relic density constraint is applied with both a lower and upper bound in all but one of these studies, and hence conclusions on the character of allowed neutralino dark matter mostly do not correspond to the present work where we allow the lightest neutralino to underpopulate the observed relic density. Finally, the list of experimental inputs included in these scans includes only a few of the measurements considered in our paper.

The closest potential comparison to our work is the MasterCode global fit of the pMSSM10~\cite{MasterCodeMSSM10}, which performs a global fit in the weak scale MSSM parameters $M_1$, $M_2$, $M_3$, $m_{\tilde{q}}$ (a unified first and second generation squark mass),  $m_{\tilde{q_3}}$, $m_{\tilde{l}}$, $A$, $\mu$, $M_A$, $\tan\beta$. Despite the clear differences in their model definition (and prior ranges on similar parameters), it is possible to note some interesting comparisons with their results, particularly in certain sparticle mass planes that are either insensitive to differences in the model definition, or have straightforward changes in behaviour based on the assumed parameter set. These are as follows:

\begin{itemize}
\item In the $\tilde{t}-\tilde{\chi}_1^0$ mass plane, we reproduce the MasterCode observation of a thin strip of $h/Z$ funnel models running parallel to the $\tilde{t}$ mass axis until $\approx 4$~TeV, with $\tilde{\chi}_1^0$ masses less than 100 GeV. We see this start at $m_{\tilde{t}_1}\approx 2$~TeV rather than the MasterCode value of $\approx 1$~TeV which is consequence of that fact that our MSSM7 model has a unified sfermion mass, rather than having separate parameters for the first/second generation squark masses, and for the slepton sector. The Higgs mass constraint pushes up the sfermion mass scale in our model in order to generate at least one stop mass that is capable of inducing large radiative corrections to the Higgs mass, leaving the other stop to be light only through large stop mixing. The prior range on the trilinear couplings then sets an effective lower bound on the lightest stop mass permissible in our model.
\item The $\tilde{\tau}_1-\tilde{\chi}_1^0$ mass plane looks very different in the two sets of results, with our 2$\sigma$ region sitting at much higher masses. This is an obvious consequence of having a unified sfermion mass scale in our scan, vs separate squark and slepton mass parameters in the MasterCode results. Our sfermions are pushed to large masses by the Higgs mass constraint, as described above. Note that this removes the stau co-annihilation region from our results. 
\item The MasterCode results show that $m_{\tilde{\chi}_1^0}\le 500$~GeV at the 95\% CL, which is attributed to the effect of the $g-2$ likelihood. In contrast we see a much larger upper bound on  $m_{\tilde{\chi}_1^0}\le 500$, extending to $\approx$ 3 TeV, with $m_{\tilde{\chi}_1^0}\le \approx 1$~TeV at the 68\% CL. Differences in the behaviour of the lightest neutralinos and charginos can almost certainly be attributed to the fact that we assumed GUT scale relations between $M_1$, $M_2$ and $M_3$, whereas these are free parameters in the MasterCode study. LHC limits on the gluino mass will therefore indirectly tend to increase the neutralino mass scale, whilst the lightest neutralino will remain predominantly bino in character in a large proportion of our parameter space. {\bf MJW: Is any of this even remotely correct?!} An increase in the neutralino mass might already place us in a region of the MSSM7 where the $g-2$ constraint is relatively poorly accommodated, with the effect that its influence on the combined likelihoods of the best fit points is minimised.
\item Discounting the increased range of neutralino masses, the rest of the features in the $\tilde{t}-\tilde{\chi}_1^0$ mass plane look qualitatively similar between our results and those of MasterCode. We see a bulk of chargino co-annihilation models extending to low neutralino masses, and ranging over all stop masses from a lower bound of $\approx$ 1 TeV. We also see a separate island running close to the $m_{\tilde{\chi}_1^0}=m_{\tilde{t}}$ line. These disparate regions are, however, distinguished by their composition. In the MasterCode results, the $m_{\tilde{\chi}_1^0}\approx m_{\tilde{t}}$ region is dominantly composed of chargino co-annihilation models, whereas we see this dominated by a mixture of stop co-annihilation, sbottom co-annihilation and the $A/H$ funnel mechanisms. The bulk region for us appears to exist with a mixture of chargino co-annihilation and the $A/H$ funnel mechanism being active, rather than the MasterCode result of chargino co-annihilation only. This is simply a plotting convention however. A close reading of the MasterCode paper reveals that, in this case, they simply plot chargino co-annihilation since it is the dominant mechanism.
\item The $m_A-\tan\beta$ plane is similar in both sets of results, with two exceptions. The first is that our 2$\sigma$ contour extends to higher values of $\tan\beta$ than the MasterCode results. This cannot be explained solely from the difference in the prior range for $\tan\beta$ ($<$70 for us, $<$60 for them). We also do not see stau co-annihilation (due to our unified sfermion mass assumption), but we do see a stop co-annihilation at low $\tan\beta$ which has not apparently been found in the MasterCode results.
\end{itemize}


\bibliography{R1}

\end{document}



